APISENS- Sentiment Scoring Tool for APIs with Crowd-Knowledge

Utilizing pre-existing software artifacts, such as libraries and Application Programming Interfaces (APIs), is crucial for software development efficiency. However, the abundance of artifacts that provide similar functionality can lead to confusion among developers, resulting in a challenge for proper selection and implementation. Through our preliminary investigation, we found that utilizing the collective knowledge of a crowd can greatly assist developers in acquiring a thorough and complete understanding of the complexities involved in the software development process. Especially as emotions are an inseparable part of human nature, it influences developers' activities. In this regard, we attempt to build a tool that can retrieve sentiment information for software APIs so that developers can determine APIs to utilize for their tasks. We employ the dataset from the most popular platforms (i.e., Twitter and YouTube) to build our research prototype. The source code, tool, and demo video are available on GitHub at \url{https://github.com/FalconLK/APISens}.

==> conclusion.tex <==
\section{Conclusion}
% This paper proposes a tool named \toolname which retrieves sentiment scores for software APIs by analyzing the crowd-knowledge.
In this paper, we propose a tool named \toolname which analyzes crowd-knowledge to determine sentiment scores for software APIs. 
Specifically, \toolname utilizes data from popular online platforms such as Twitter and YouTube to extract sentiment scores from discussions and videos related to the APIs in question. 
Based on our investigation of user experience, we observe that our tool has the potential to be a useful tool for API comprehension.
Furthermore, we suggest prospective ideas to improve the tool for the research community.
In the future, we plan to integrate more features to practically support developers.
We release the source code and the demo video of \toolname at https://github.com/FalconLK/APISens.
